Multiblock Grid Generation for Simulations in Geological Formations

Simulating fluid flow in geological formations requires mesh generation, lithology mapping to the cells, and computing geometric properties such as normal vectors and volume of cells. The purpose of this research work is to compute and process the geometrical information required for performing numerical simulations in geological formations. We present algebraic techniques, named Transfinite Interpolation, for mesh generation. Various transfinite interpolation techniques are derived from 1D projection operators. Many geological formations such as the Utsira formation (Torp and Gale, 2004; Khattri, Hellevang, Fladmark and Kvamme, 2006) and the Snohvit gas field (Maldal and Tappel, 2004) can be divided into layers or blocks based on the geometrical or lithological properties of the layers. We present the concept of block structured mesh generation for handling such formations.

==> Makefile <==
# Generic make file for LaTeX: requires GNU make
#
# This makefile provides four targets: dvi, ps, pdf and clean.
# The default is "pdf".
# To make a dvi file, type "make dvi"
# To make a ps file, type "make ps".
# To make a pdf file, type "make pdf" or simply "make".
# To remove all files generated by make, type "make clean".
#
# Rouben Rostmaian
# September 2002

TEXFILE =   article.tex
#TEXFILE	= slides.texTPFA_diagonal_perm_variable.tex

.PHONY: dvi ps pdf clean

pdf:	$(TEXFILE:.tex=.pdf)
ps:	$(TEXFILE:.tex=.ps)
dvi:	$(TEXFILE:.tex=.dvi)

%.dvi: %.tex
	( \
	\latex $<; \
	while \grep -q "Rerun to get cross-references right." $(<:.tex=.log); \
	do \
		\latex $<; \
	done \
	)

%.ps: %.dvi
	\dvips -q -t a4 $<

%.pdf: %.ps
	\ps2pdf -dPDFSETTINGS=/prepress $<

clean:
	@\rm -f \
	$(TEXFILE:.tex=.aux) \
	$(TEXFILE:.tex=.log) \
	$(TEXFILE:.tex=.out) \
	$(TEXFILE:.tex=.dvi) \
	$(TEXFILE:.tex=.ps)

